WorldModelBench: Judging Video Generation Models As World Models

Video generation models have rapidly progressed, positioning themselves as video world models capable of supporting decision-making applications like robotics and autonomous driving. However, current benchmarks fail to rigorously evaluate these claims, focusing only on general video quality, ignoring important factors to world models such as physics adherence. To bridge this gap, we propose WorldModelBench, a benchmark designed to evaluate the world modeling capabilities of video generation models in application-driven domains. WorldModelBench offers two key advantages: (1) Against to nuanced world modeling violations: By incorporating instruction-following and physics-adherence dimensions, WorldModelBench detects subtle violations, such as irregular changes in object size that breach the mass conservation law - issues overlooked by prior benchmarks. (2) Aligned with large-scale human preferences: We crowd-source 67K human labels to accurately measure 14 frontier models. Using our high-quality human labels, we further fine-tune an accurate judger to automate the evaluation procedure, achieving 8.6% higher average accuracy in predicting world modeling violations than GPT-4o with 2B parameters. In addition, we demonstrate that training to align human annotations by maximizing the rewards from the judger noticeably improve the world modeling capability. The website is available at https://worldmodelbench-team.github.io.

==> sec/6_limitation.tex <==
\section{Limitation}
The paper scopes in accessing the video generation models in its ability to simulate the real-world dynamics. However, this is not the only measure that a video generation model can be useful. For example, the ability to create impossible interactions, such as fire flaming inside water might have potential applications such as in creative arts.


==> sec/tables/table1_rm_acc_comparison.tex <==
%\begin{figure}[h]
%    \centering
%\includegraphics[width=0.5\textwidth]{sec/figures/UI.png}
%    \caption{Human annotation interface.}
%    \vspace{-15pt}
%    \label{fig:human_interface}
%\end{figure}

==> sec/tables/table3_video_benchmark.tex <==
\begin{tabular}{lll}
\toprule
\textbf{Model} & \textbf{Instruction (\%) $\uparrow$} & \textbf{Physics (\%) $\uparrow$} \\
\quad+\textit{Method} & \textbf{following} & \textbf{Adherence} \\
\midrule
\texttt{GPT-4o} & 69.2 & 57.1 \\
\textit{\quad+CoT} & 65.2 & \textbf{85.4} \\
\texttt{Gemini-1.5-Pro} & 51.5 & 50.0 \\
\textit{\quad+CoT} & &  \\
\texttt{Qwen2-VL-72B} &  &  \\
\midrule
\texttt{Qwen2-VL-2B} & 67.2 & 36.4 \\
\texttt{VILA-2B}\textit{ +Zero-Shot} & 66.7 & 50.5 \\
\texttt{VILA-2B}\textit{ +Fine-tuned} & \textbf{70.2} & 69.7 \\
\bottomrule
\end{tabular}

==> sec/tables/table5_vbench.tex <==
\begin{table}
%\begin{wraptable}{r}{0.5\linewidth}
% \vspace{-7mm}
% \begin{table}[htbp]
\begin{center}
% \dacheng{Relationship between different dimensions}
\caption{Spearman coefficient between different category of our benchmark versus others.\dacheng{@Shuo}}%\dacheng{add CoT to our model capability; we want to show our is better than GPT4-o} .}
\begin{tabular}{lll}
\toprule
\textbf{Category} & \textbf{VBench} & \textbf{FVD}\\
\midrule
\texttt{Instruction} &  &  \\
\texttt{Common Sense} &  &  \\
\texttt{Physics Adherence} & & \\
\texttt{Total} &  & \\
\bottomrule
\end{tabular}
\end{center}
\label{tab:correlation}
% \end{table}
%\end{wraptable}
\end{table}
